OTW: Optimal Transport Warping for Time Series

Dynamic Time Warping (DTW) has become the pragmatic choice for measuring distance between time series. However, it suffers from unavoidable quadratic time complexity when the optimal alignment matrix needs to be computed exactly. This hinders its use in deep learning architectures, where layers involving DTW computations cause severe bottlenecks. To alleviate these issues, we introduce a new metric for time series data based on the Optimal Transport (OT) framework, called Optimal Transport Warping (OTW). OTW enjoys linear time/space complexity, is differentiable and can be parallelized. OTW enjoys a moderate sensitivity to time and shape distortions, making it ideal for time series. We show the efficacy and efficiency of OTW on 1-Nearest Neighbor Classification and Hierarchical Clustering, as well as in the case of using OTW instead of DTW in Deep Learning architectures.

==> sections/fc_vs_otnet.tex <==
\subsection{Fully Connected architecture vs OT-Net on real datasets}
After concluding that the computational bottleneck in DTW-Net means it is not a feasible approach for classification on real datasets, we turn to compare OT-Net with a Fully Connected architecture. the hidden layer sizes for OT-Net and the Fully connected network are set as $[500, 500, 500]$. The results are summarized in \ref{tab:fc-vs-otnet-comparison}.

We observe that our OT-Net outperforms only in a few types of datasets, namely, Image, traffic and Power-type datasets. Of these three types, only the Image datasets have a large amount of examples to draw a strong conclusion. In any case, architectures like CNNs or Transformers might be more suitable for such kind of data. For this reason it might make more sense to combine OT-layers with Convolutional Layers, or explore attention-based mechanisms using Optimal Transport instead of inner products. Such alternatives are outside the scope of this work but constitute a promising avenue of research. For Traffic and Power datasets OT-Net and OT-based methods seem to outperform the baselines throughout all our experiment, but further confirmation with similar datasets is needed to draw a strong conclusion. Currently, we are unaware of more public benchmark datasets with similar characteristics.

\begin{table}
\centering
\begin{tabular}{c c c c}
{\bf Dataset Type} & \textbf{Total Datasets} & \textbf{OT-Net improves over FC} & \textbf{Percentage}  \\ \hline
Image        & 18 & 27 & \textbf{66.66} \\
Spectro      & 5  & 11 & 45 \\
Sensor       & 7  & 17 & 41.17 \\
Device       & 2  & 6  & 33.33 \\
Medical Data & 3  & 12 & 25 \\
Traffic      & 2  & 2  & \textbf{100} \\
Power        & 1  & 1  & \textbf{100} \\
all          & 38 & 76 & 50 \\ \hline

\end{tabular}
\caption{Number of datasets in the UCR time-series benchmark collection (and percentage) where OT-Net classification outperforms the Fully Connected network alternative. The metric used is the error on the test set. Results split by dataset type. Noticeable improvements in boldface.}
\label{tab:fc-vs-otnet-comparison}
\end{table}

==> sections/schedule.tex <==
\begin{table}
\centering
\begin{tabular}{r c c c c c}
Week         & Sec. 3 (Theory) & Exp. 4.1 & Exp. 4.2 & Exp. 4.3 & Writing \\ \hline
2/28 - 3/4   & \cmark          & \cmark   & -        & -        & -       \\
3/7 - 3/11   & \cmark          & \cmark   & -        & -        & -       \\
3/14 - 3/18  & \cmark          & \cmark   & \cmark   & -        & -       \\
3/21 - 3/25  & -               & \cmark   & \cmark   & -        & -       \\
3/28 - 4-1   & -               & -        & \cmark   & \cmark   & -       \\
4/4 - 4/8    & -               & -        & \cmark   & \cmark   & -       \\
4/11 - 4/15  & -               & -        & -        & \cmark   & \cmark  \\
4/18 - 4/22  & -               & -        & -        & \cmark   & \cmark  \\
4/25 - 4/29  & -               & -        & -        & -        & \cmark 
\end{tabular}
\end{table}

